Near-Optimal Online Multiselection in Internal and External Memory

We introduce an online version of the multiselection problem, in which q selection queries are requested on an unsorted array of n elements. We provide the first online algorithm that is 1-competitive with Kaligosi et al. [ICALP 2005] in terms of comparison complexity. Our algorithm also supports online search queries efficiently. We then extend our algorithm to the dynamic setting, while retaining online functionality, by supporting arbitrary insertions and deletions on the array. Assuming that the insertion of an element is immediately preceded by a search for that element, we show that our dynamic online algorithm performs an optimal number of comparisons, up to lower order terms and an additive O(n) term. For the external memory model, we describe the first online multiselection algorithm that is O(1)-competitive. This result improves upon the work of Sibeyn [Journal of Algorithms 2006] when q > m, where m is the number of blocks that can be stored in main memory. We also extend it to support searches, insertions, and deletions of elements efficiently.

==> conclusion.tex <==
\section{Discussion}
\label{sec:comp-past-future}

% \subsection{Our Results}
% \label{sec:our-results}

Our results can be summarized as follows:
\begin{itemize}
\item We generalized the multiselect problem defined by Dobkin and
  Munro~\cite{dobkin-multiselect} to
  \begin{itemize}
  \item the online context where the queries are given one by one in
    any order (as opposed to a cluster of queries sorted),
  \item multisets (as opposed to sets where no value is repeated), and
  \item select, rank and search queries (as opposed to only select
    queries).
  \end{itemize}

\item In Main Memory, we gave
  \begin{itemize}
  \item an $\Oh(1)$-competitive online algorithm to solve select, rank
    and search queries over $N$ non ordered values in time
    $4N\entropy(\Delta_1,\ldots,\Delta_q)$ using $N+\Oh(\lg N)$ bits
    of working space, where $(\Delta_1,\ldots,\Delta_q)$ is the
    sequence of gaps between the positions hit by the $q$
    queries. This complexity is within a constant factor of the lower
    bound shown by Munro and Dobkin~\cite{dobkin-multiselect} for the
    offline version of the problem; and
  \item an $\Oh(1)$-competitive online algorithm to solve select, rank
    and search queries over $N$ non ordered values in the same time,
    but space $\Oh((\lg N)^2)$ when the queries arrive in monotone
    order.
  \end{itemize}

\item In External Memory,
  \begin{itemize}

  \item we showed a lower bound of $n\log_m n - \sum_{i\in q}
    \delta_i\log_m\delta_i$ (which we note
    $n\entropy_m(\delta_1,\ldots,\delta_q)$ for short) on the number
    of accesses required in order to solve $q$ select queries over $n$
    pages of data given $m$ pages of local memory, where
    $(\delta_1,\ldots,\delta_q)$ is the vector formed by the number of
    pages between the pages hit by the $q$ queries; and gave

  \item an $\Oh(1)$-competitive online algorithm to solve select, rank
    and search queries over $n$ non ordered pages in
    $\Oh(n\entropy_m(\delta_1,\ldots,\delta_q))$ accesses; which implies

  \item an offline algorithm improving on the multiselect solution
    described by Sibeyn~\cite{sibeyn:external-selection} on instances
    where the positions hit by the queries are irregularly spaced.

  \end{itemize}
\end{itemize}

All our results are within a constant factor of less than $4$ of the
optimal, for a fixed sequence of queries, in the worst case over all
instances of $N$ elements. 
%
% \subsection{Future Work and Open Problems}
% \label{sec:future-work-open}
%
Following on this work we are considering the following problems:

\begin{enumerate}

\item reducing the constants involved (which are nevertheless no
  larger than $4$), in order to yield among other things,
  \begin{itemize}
  \item online algorithms in Main Memory still performing in time
    $\Oh(N\entropy(\Delta_1,\ldots,\Delta_q))$, but only
    $N\entropy(\Delta_1,\ldots,\Delta_q)$
    $+o(N\entropy(\Delta_1,\ldots,\Delta_q))+\Oh(N)$ comparisons; and
  \item an online algorithm in External Memory performing
    $n\entropy_m(\delta_1,\ldots,\delta_q)$ $+o(n\entropy_m(\delta_1,\ldots,\delta_q))+\Oh(n)$
    memory accesses;
  \end{itemize}

\item merging our two algorithms into a single one, which is at once
  optimal in Main Memory and in External Memory;

\item taking advantage of repetitions in the input (e.g. if $A$
  contains only $\sigma$ distinct values);

\item taking advantage of pre-existing order in the input (e.g. if $A$
  already contains sorted subsequences, or if $A$ is already
  partitioned, which results in a small number of inversions);

\item considering other memory models such as Flash memory, where the
  dissymetry between reading and writing should require a distinct
  treatment from External Memory yet yield interesting results (given
  the example of Sibeyn's proposal~\cite{sibeyn:external-selection}
  performing more reads in order to reduce the number of writes).

\end{enumerate}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper"
%%% End: 


==> defs.tex <==
\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}

\def\id#1{\ensuremath{\mathit{#1}}}
\let\idit=\id
\def\idbf#1{\ensuremath{\mathbf{#1}}}
\def\idrm#1{\ensuremath{\mathrm{#1}}}
\def\idtt#1{\ensuremath{\mathtt{#1}}}
\def\idsf#1{\ensuremath{\mathsf{#1}}}
\def\idcal#1{\ensuremath{\mathcal{#1}}}  % Calligraphy style (caps only)

% This defines \cramped, which reduces whitespace around \item
% "Cramped" list style, put after \begin{itemize}
\def\cramped 
  {\parskip\@outerparskip\@topsep\parskip 
  \@topsepadd2pt\itemsep0pt}

% The proof environment. For proofs that don't start with ''Proof:''
% use the proofarg environment with the desired start as argument.
%\newenvironment{proof}{\trivlist\item[]\emph{Proof}:}%
{\unskip\nobreak\hskip 1em plus 1fil\nobreak$\Box$
\parfillskip=0pt%
\endtrivlist}
\newenvironment{proofsketch}{\trivlist\item[]\emph{Proof Sketch}:}%
{\unskip\nobreak\hskip 1em plus 1fil\nobreak$\Box$
\parfillskip=0pt%
\endtrivlist}
\newenvironment{proofarg}[1]{\trivlist\item[]\emph{#1}:}%
{\unskip\nobreak\hskip 2em plus 1fil\nobreak$\Box$
\parfillskip=0pt%
\endtrivlist}
\newenvironment{proofof}[1]{\trivlist\item[]{\em Proof of #1\/}:}%
{\unskip\nobreak\hskip 2em plus 1fil\nobreak$\Box$
\parfillskip=0pt%
\endtrivlist}

% These are the end boxes for the proof environment
\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern3pt
  \vbox{\kern3pt#1\kern3pt}\kern3pt\vrule}\hrule}}
\def\Box{\boxit{\null}}

\newcommand{\zero}{\idbf{0}}
\newcommand{\one}{\idbf{1}}
\newcommand{\A}{\texttt{A}}
\newcommand{\B}{\texttt{B}}
\newcommand{\select}{\id{select}}
\newcommand{\search}{\id{search}}
\newcommand{\rank}{\id{rank}}
\newcommand{\rankzero}{\id{rank}_\zero}
\newcommand{\rankone}{\id{rank}_\one}
\newcommand{\selectzero}{\id{select}_\zero}
\newcommand{\selectone}{\id{select}_\one}
\newcommand{\rankb}{\id{rank}_b}
\newcommand{\selectb}{\id{select}_b}
\newcommand{\flip}{\id{flip}}

\newcommand{\ins}{\id{insert}}
\newcommand{\delete}{\id{delete}}
\newcommand{\del}{\id{delete}}
\newcommand{\indel}{\id{indel}}

\newcommand{\qselect}{\id{qselect}}
\newcommand{\qsearch}{\id{qsearch}}
\newcommand{\qselectIO}{\id{qselect}}
\newcommand{\qsearchIO}{\id{qsearch}}


==> merge.tex <==
\newcommand{\B}{\mathcal{B}}

\section{Merging Costs}

Our goal here is to show that, for each array element in an interval,
it participates in $1+o(1)$ comparisons to perform merges before
the pivot selection and partitioning operations done to move to the
next smaller interval.

Let our current interval have length $\Delta$, recursion depth $d$,
and run length bound $l=1+\lfloor \lg d \rfloor$, so that $l$
increases by one when the recursion depth doubles.

Consider a run of length $s+t$ which splits over the pivot into
runs of length $s$ to the left and $t$ to the right with $s\le t$.
Compute integers $k$ and $s_r$ such that $s=2^{-k}l+s_r$ with
$k$ as small as possible (so that $s_r<s/2$, and $s\le l/2^{k-1}$).
A run of length $s$ must merge $k$ times to obtain a run of length
at least $l$.
In the process, $(k-1)s$ comparisons beyond the desired one comparison
per element bound are performed.

If $t\ge l$, the other half of the run is not merged, giving us an excess of
$t\ge l$ element comparisons that are not used at this recursion depth.
$(k-1)s \le (k-1) 2^{-(k-1)}l \le l \le t$ and so the total number
of comparisons is no more than one per element for this run.

So we can assume $t<l$ so that it is merged once using $t$
comparisons.
We will bound the excess $(k-1)s$ comparisons from the one side
using \textit{excess length} on both sides.
The excess length of an interval is the sum over lengths of runs $v>l$
of $v-l$.
The run of length $t$ merges to form a run of length
$2t\ge 2l-2s$ which has excess length of at least $2l-s$, and
this run ``owns'' half of this, or $l-s/2$.
But this is larger than $(k-1)s$.

Next we observe that if $s+t>l$, if we write $s+t=l+x$ so that
$x$ was excess length from the parent interval, we did not need to use
any of the inherited excess length $x$ to bound the $(k-1)s$ extra
comparisons at this level.  Thus, the $x$ excess length is preserved.
Therefor, we can bound all the excess comparisons done by the algorithm
by bounding the total excess length of all intervals that are either
leaves, or are not partitioned; the unpartitioned ones we count the
excess as if we had performed the merges in them (even though we don't).
It is then easy to see the sum total of the excess lengths must be
$O(n)$.



==> previousWork.tex <==
%\section{Previous Work}


\subsection{Selection in Main Memory}
\label{sec:ram-model}

%\paragraph{Median algorithms}

Hoare~\cite{hoare:quickselect} proposed an expected linear time algorithm for the selection problem. 
%
Blum~\etal~\cite{blum:median} designed a deterministic algorithm to find the median
of a given set of elements (and hence also for the selection problem)
in linear number of comparisons in the worst-case.
%
The comparison complexity of this algorithm was improved by
Sch{\"o}nhage~\etal~\cite{schonhage:median} to $3N+o(N)$, and further
to at most $2.942 N + o(N)$ by Dor and Zwick~\cite{dor:median-upperbound}.


%\paragraph{$\Oh(N)$ rank and select}

A generalization of the median is the operator $\select(A,i,j,r)$
which selects the element of any specified rank $r$ in any range of
positions $[i..j]$ in $A$ $\forall r,i,j\in[1..N]$ (as opposed to the
element of rank $\lfloor {(j-i+1)/2}\rfloor$ for the median).
%
A linear time algorithm for median immediately yields a linear time
algorithm for selection~\cite{hoare:quickselect}.

The inverse of $\select$ is the $\rank(A,i,j,x)$ operator which
returns the number of elements strictly smaller than $x$, plus one
(effectively the position of $x$ in $A$ once sorted, if $x$ is in
$A$). This is obviously supported in $j-i+1$ comparisons my merely
scanning the interval.

%\begin{INUTILE}
%  The main interest of such operators is to partition the input into
%  two parts, such that all elements of the first part are smaller than
%  all the elements of the second part. We combine this partitioning
%  with the previous operators as $\rangePartitionSelect(A,i,j,r)$,
%  $\rangePartitionRank(A,i,j,x)$, and
%  $\rangePartitionSearch(A,i,j,x)$.
%%
%  Given support for $\select(A,i,j,r)$ in $2.942(j-i+1)+o(j-i+1)$
%  comparisons, adding
%\end{INUTILE}


%\paragraph{$\Oh(N\entropy(\Delta))$ Offline Multiselect}

In 1971, Chambers~\cite{chambers:partialsort} proposed a modification
to the Quicksort algorithm~\cite{hoare:quicksort} to solve a sequence of 
select queries, introducing the notion of {\em partial sorting}.
Given an unsorted array $A$, and a set $S = \{ s_1, \dots, s_q\}$ of $q$
select queries, the partial sorting procedure rearranges the elements of $A$ 
such that the following condition is true for all elements $s_i \in S$:
for $1 \le j < s_i, A[j] \le A[s_i]$ and for $ s_i < j \le n, A[j] \ge A[s_i]$.
%In other words, all the elements in $Q$ are placed in their correct positions 
%in the sorted order after the partial sort, and array is "partitioned" such that 
%all the elements smaller than $q_i$ are to the left of ....

In 1984 Dobkin and Munro~\cite{dobkin-multiselect} showed a lower
bound of $N\entropy(\Delta)$ on the number of comparisons required to
answer $q$ queries hitting positions in $A$ separated by intervals of
respective sizes forming the vector $\Delta \equiv
(\Delta_1,\ldots,\Delta_q)$, and gave an asymptotically optimal
algorithm answering the $q$ queries using $3N\entropy(\Delta)$
comparisons, and $\Oh(N\entropy(\Delta))$ time.
%\begin{TODO}
%  CHECK the constant $3$: Shouldn't it be $4$ or higher, if the Median
%  is already with constant of $3$ and partitioning is with constant of
%  $1$? -- 
%  SSR: May be the median finding can be combined with the 
%  partitioning. Any median algorithm has to compute the ranks of some
%  elements (median of medians). The partitioning step can be easily 
%  combined with the rank computation step. So, may be our simple 
%  algorithm can also achieve a constant of 3, if we combine the 
%  median finding with partitioning.
%\end{TODO}


%\begin{optimallyCompetitiveRAM}
  %\paragraph{$NH+o(NH)+\Oh(N)$ cmps offline multiselect}

  In 2006, Kaligosi~\etal~\cite{kaligosi-multiselect} reduced the
  number of comparisons performed to
  $N\entropy(\Delta)+o(N\entropy(\Delta))+\Oh(N)$,
  still within time $\Oh(N\entropy(\Delta))$,
  approximating the median of blocks in $A$ by the median of the
  middles of runs in $A$, of size carefully chosen and maintained.

%\end{optimallyCompetitiveRAM}


%\begin{TODO}
%  HIGHLIGHT the definition of rank and select queries on arrays
%  containing repetitions: it is as simple as counting with multiplicity
%  and the definitions above should still work, but it is worth
%  pointing out to the reader.
%\end{TODO}


\subsection{External Memory model}
\label{sec:external-memory}

%\paragraph{ External Memory model: $B$, $M$, $n$ and $m$.}
We also consider the online multiselect problem in the \emph{external
memory model} proposed by Aggarwal and Vitter~\cite{aggarwal-iomodel}.
In this model, data is transferred between the disk and the main memory 
(i.e., read from the disk to the main memory, and written to the disk from 
the main memory) in chunks of size $B$ elements. Each such transfer is referred to 
as an I/O. The model assumes an external disk of unbounded capacity, and a
main (internal) memory of limited capacity, $M$ data elements or $m \equiv M/B$ blocks.
The performance measures of an algorithm are: the space, which is the 
number of blocks on disk that are used by the algorithm to store data, and 
time, which is the number of I/Os performed during the algorithm.

%\paragraph{ word RAM model in external memory}
In addition to Aggarwal and Vitter's parameterization of the model, we
will also consider the number of bits $w$ occupied by an element. This
is required in order to evaluate the space taken by a bit vector where
each bit corresponds to a single element.

%\paragraph{ External Merge Sort in $2n\lceil\log_m n\rceil$ accesses }

In this model, Aggarwal and Vitter~\cite{aggarwal-iomodel} showed that
a given unsorted array $A$ of length $N$ stored on the disk in $n
\equiv N/B$ blocks can be sorted using the \emph{external merge sort}
algorithm in $O(n \log_m n)$ I/Os.

%\paragraph{ Comparison of traditional median algorithm with optimal external sorting}

Sibeyn~\cite{sibeyn:external-selection} considered the selection
problem in the external memory model.
%
He observed that the recursive `median-of-medians'
algorithm of Blum~\etal~\cite{blum:median}, adapted to 
the external memory,
is outperformed by the external merge sort algorithm
for most practical values of $n$ and $m$:
the first one performs $12 n$ I/Os which is more than the 
$n\log_m n$ I/Os performed by the external merge sort,
as long as $n<m^{12}$, a condition which holds for all practical 
values of $n$ and $m$.

%\paragraph{ $n+o(n)$ accesses for median, rank and select in External memory}

Sibeyn~\cite{sibeyn:external-selection} presented an alternative algorithm
to select the $r$-th element with much less external accesses, without
modifying the original array $A$ but writing in external
memory, a hierarchy of summaries of $A$.
%
This ``index construction phase'' is independent of the queries,
and is the most time consuming operation, taking $n + o(n)$ accesses.
%
Since the rank of an element in $A$ can be approximated
through its rank in the summaries, this permits 
%
to compute an interval of candidate elements from the summaries only
(without accessing the main data), and in turn
%
to focus only on the pages matching this interval, 
%
within $o(n)$ additional accesses.
%
%\begin{LONG}
%  His solution comes in two variants, corresponding to two different
%  trade-offs in terms of the amount of reading and writing performed
%  in external memory.
%\end{LONG}
%

%%\paragraph{ $f(q,n)$ accesses for multiselect, both offline and online}

Sibeyn observed that his result can be \emph{easily generalized to
  solve offline multiselect queries}, and also in the
\emph{online} setting where the queries are given one-by-one.
%
More specifically, as the index construction phase of his 
selection algorithm is independent of the query, 
the index can be used to answer any number of queries
-- using an additional $o(n)$ accesses for each query.
%
Thus, it provides a solution to the online multiselect problem in 
external memory.
%
Yet, Sibeyn's solution is optimal only in the worst case over all
sequences of $q$ queries: they can be outperformed when the queries
are irregularly spaced.
%\begin{JEREMY}
%  Isn't his solution suboptimal when there are more than $N\lg N$
%  select queries, and it would be better to sort the input and then
%  answer each select query in exactly one access?
%  SSR: I guess, by $N$, you mean the number of blocks (and not the number 
%  of elements)..?
%  SSR: I think, his solution is suboptimal even for $N$ (or less) select queries.
%  After the preprocessing step, he's not modifying the index while answering 
%  the queries. So, even what we say above ("his solution is optimal
%  only in the worst case over all sequences ...") is probably wrong.
%\end{JEREMY}
%
%\begin{INUTILE}
%  \begin{LONG}
%    \subsection{Online Select, Rank and Search queries}
%    \label{sec:online-select-rank-2}
%
%    % \paragraph{ Definition of Online algorithm}
%
%    % \paragraph{ Definition of Competitive Ratio}
%
%    % \paragraph{ Definition of Online Select, Rank and Search
%    % queries}
%
%  \end{LONG}
%\end{INUTILE}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../paper"
%%% End: 

